Unified Questioner Transformer for Descriptive Question Generation in Goal-Oriented Visual Dialogue

Building an interactive artificial intelligence that can ask questions about the real world is one of the biggest challenges for vision and language problems. In particular, goal-oriented visual dialogue, where the aim of the agent is to seek information by asking questions during a turn-taking dialogue, has been gaining scholarly attention recently. While several existing models based on the GuessWhat?! dataset have been proposed, the Questioner typically asks simple category-based questions or absolute spatial questions. This might be problematic for complex scenes where the objects share attributes or in cases where descriptive questions are required to distinguish objects. In this paper, we propose a novel Questioner architecture, called Unified Questioner Transformer (UniQer), for descriptive question generation with referring expressions. In addition, we build a goal-oriented visual dialogue task called CLEVR Ask. It synthesizes complex scenes that require the Questioner to generate descriptive questions. We train our model with two variants of CLEVR Ask datasets. The results of the quantitative and qualitative evaluations show that UniQer outperforms the baseline.

==> secs/algo.tex <==
\begin{algorithm}[t]
% \setstretch{1.2}
\SetAlgoLined
\SetKwIF{If}{ElseIf}{Else}{if}{:}{elif}{else:}{end}
{\footnotesize
\LinesNumbered
\KwData{$\mathcal{O}$}
% \KwResult{$G’=(X,V)$ with $V\subseteq U$ such that $G’^{tc}$ is an interval order.}
% $\triangleright$ initialization \\
% loop for one scene
The Oracle picks an goal object $o^{*} \in \mathcal{O}$ \\
q = [], a = []  \hfill $\triangleright$ questions $\&$ answers \\
\For(\hfill $\triangleright$ dialogue loop){$t=1$ \KwTo $T$}{
    $\triangleright$ Prepare embeddings  \hfill $\triangleright$ see \S\redr{4.1}\\
    $\bm{x}_{v} \leftarrow \mathcal{F}_{v}([\bm{o}_{v}(i), \bm{o}_g^{\mathcal{N}}(i)]_{i\in \mathcal{N}})$\\
    $\bm{x}_{l}^{t} \leftarrow{} [\mathrm{[CLS]}, w_1^1, w_2^1,..., w_{W_1}^1, a^1, w_1^{2}, ..., a^{t-1}]$ \\
    $\bm{x}_{h} \leftarrow [\bm{x}_{v}, \bm{x}_{l}^{t}]$  \\
    $\bm{x}_{e} \leftarrow \bm{x}_{h} + \bm{x}_{\mathrm{seg}} + \bm{x}_{\mathrm{pos}}$  \\

    $\triangleright$ \oet{} \hfill $\triangleright$ see \S\redr{4.2}\\
    $\{\tilde{\mathcal{X}}_{o}, \tilde{X}_{[\rm CLS]}, \tilde{\mathcal{X}}_{l}\} \leftarrow \oet{}(\bm{x}_{e})$ \\
    $\sigma_{o} \leftarrow [\mathrm{sigmoid}(\mathcal{F}_{o}(\tilde{X}_{o}^{i}) \cdot \mathcal{F}_{c}(\tilde{X}_{[\rm CLS]}))]_{i \in\mathcal{N}}$\\
    ${P}_{\hat{o}} \leftarrow \mathrm{softmax}(\sigma_o)$\\

    % OTM
    $\triangleright$ \otgt{} \hfill $\triangleright$ see \S\redr{4.3}\\
    Get top-k object ids: $\mathcal{K} \leftarrow \mathrm{argtopk}({P}_{\hat{o}})$ \\
    % prepare top-k features
    % $\bm{x}_{k} = [\bm{o}_{v}(i), \bm{o}_{g}(i), \bm{o}_{g}(i, j), {P}_{\hat{o}}(i)]_{(i, j) \in \mathcal{K}}$ \\
    $\bm{x}_{k} \leftarrow [\mathcal{F}_{A}(\bm{o}_{v}(i)), \mathcal{F}_{B}(\bm{o}_{g}^{\mathcal{K}}(i)), \mathcal{F}_{C}({P}_{\hat{o}}(i))]_{i \in \mathcal{K}})$ \\
    % $\bm{\hat{g}}_k \leftarrow \mathrm{softmax}(\mathcal{F}_{l}(\mathrm{concat}[\mathcal{F}_{\mathrm{GRU}}(\bm{x}_{k})]))$ \\
    $A_t \leftarrow \mathrm{sampling}(\mathcal{F}_{\mathrm{RL}}(\bm{x}_{k}))$\\
    % $\bm{\hat{g}_k}_{base3} = \mathrm{ternary}(\mathrm{argmax}(\bm{\hat{g}_k})) \hfill \triangleright~\text{size k}$\\
    $\bm{g}_{k} \leftarrow \mathrm{ternary}(A_{t}) \hfill \triangleright~\bm{g}_k \in \mathbb{R}^{3 \times k}$\\
    $\bm{g} \leftarrow \mathrm{padding}(\bm{{g}}_{k}) \hfill \triangleright~\bm{g} \in \mathbb{R}^{3 \times \mathcal{N}}$ \\

    \uIf({\hfill $\triangleright$ end of dialogue (EOD)})
    {$A_t \in \{0, 3^{k} - 1\}$}{
        $r(S_t, A_t) \leftarrow
        \begin{cases}
            1 - r_{d}(t) & \text{if}~\mathrm{argmax}(P_{\hat{o}})==o^{*}_{id} \\
            0 & \text{otherwise}
        \end{cases}
        $\\
        break
    }
    \uElseIf({\hfill $\triangleright$ EOD should have been generated}){$t == T$}{
        % if <EOD> is not generated --> cannot acquire rewards
        $r(S_t, A_t) \leftarrow 0$\\
    }
    \Else{
        $\triangleright$ \qdt{} \hfill $\triangleright$ see \S\redr{4.4}\\
        $\mathcal{M} \leftarrow \tilde{\mathcal{X}}_{o} + \mathcal{F}_{s}(\bm{g})$ \\
        $[w_1^t, w_2^t, ..., w_{W_t}^t] \leftarrow \mathrm{\qdt{}}(\mathrm{[BOS]}, \mathcal{M})$ \\
        append $[w_1^t, w_2^t, ..., w_{W_t}^t]$~to~q, ~$a^t$~to~a \\
    }
}
\caption{\propmodel{} RL flow for a scene}
\label{alg:Algo}
}
\end{algorithm}


==> tables/results_fs.tex <==
\begin{table}[]
\footnotesize
\begin{centering}
  \begin{tabularx}{.47\textwidth}{@{}p{1.45cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}@{}}
    \toprule
%                & \multicolumn{3}{c}{Task Success (\%)} \\ \midrule
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ask3}                 & \multicolumn{2}{c}{Ask4}                                                      \\ \midrule
    Model                & New Img$\uparrow$ & New Obj$\uparrow$ & \multicolumn{1}{l}{New Img$\uparrow$} & \multicolumn{1}{l}{New Obj$\uparrow$} \\ \midrule
    % Ours (rand) & $1.73_{\pm 0.12}$  & $1.64_{\pm{0.21}}$ & $1.61_{\pm 0.07}$  & $1.72_{\pm{0.10}}$ \\
    Baseline(fs) & $59.78_{ \pm 5.75 } $ & $60.37_{ \pm 5.71 }$ & $64.76_{ \pm 1.26 } $ & $65.02_{ \pm 1.22 }$ \\
    Ours(full-fs) & $85.06_{ \pm 1.55 } $ & $85.17_{ \pm 1.47 }$ & $83.08_{ \pm 0.69 } $ & $83.70_{ \pm 0.88 }$ \\
    % Ours (SA) & $84.23_{\pm 3.93}$ & $84.04_{\pm 3.93}$ & $83.80_{\pm 0.83}$ & $83.43_{\pm 0.83}$ \\  \midrule % self attention 
    % \midrule
    \bottomrule
  \end{tabularx}
  \caption{
    Comparative results on the task success ratio
    for the baseline and \propmodel{} in reinforcement learning on stop condition.
    In stop condition, a submission action is not required and the goal object prediction is
    automatically sent to the oracle at the end of the dialogue.
}\label{tab:results_fs}
\end{centering}
\vspace{-1em}
\end{table}

% ask3_uniqer_rl_fs: $85.06_{ \pm 1.55 } $ & $85.17_{ \pm 1.47 }$ \\
% a3blfs: $59.78_{ \pm 5.75 } $ & $60.37_{ \pm 5.71 }$ \\
% ask4_uniqer_rl_fs: $83.08_{ \pm 0.69 } $ & $83.70_{ \pm 0.88 }$ \\
% a4blfs: $64.76_{ \pm 1.26 } $ & $65.02_{ \pm 1.22 }$ \\

==> tables/results_vocab.tex <==
\begin{table}[]
\footnotesize
\begin{centering}
 \begin{tabularx}{.47\textwidth}{@{}lcccc@{}}
 \toprule
                          & \multicolumn{2}{c}{Question Mean ($n_\mathrm{vocab}$)}
                          & \multicolumn{2}{c}{Dialogue Mean ($\overline{n}_\mathrm{vocab}$)} \\ \midrule
 Model & New Img   & New Obj  & New Img & New Obj \\ \midrule
 \multicolumn{1}{c}{Ask3} &                    &                  &                   &                  \\ \midrule
 Baseline   & $1.48_{ \pm 0.27 } $ & $1.48_{ \pm 0.27 }$   &    $3.15_{ \pm 0.08 } $ & $3.15_{ \pm 0.07 }$ \\
Ours(v)    & $2.62_{ \pm 0.04 } $ & $2.58_{ \pm 0.08 }$   &    $3.54_{ \pm 0.13 } $ & $3.54_{ \pm 0.16 }$ \\
Ours(num)  & $1.54_{ \pm 0.04 } $ & $1.52_{ \pm 0.03 }$   &    $2.92_{ \pm 0.11 } $ & $2.98_{ \pm 0.12 }$ \\
Ours(nu)   & $1.51_{ \pm 0.02 } $ & $1.47_{ \pm 0.07 }$   &    $3.11_{ \pm 0.17 } $ & $3.12_{ \pm 0.12 }$ \\
Ours(full) & $3.32_{ \pm 0.16 } $ & $3.35_{ \pm 0.08 }$   &    $3.82_{ \pm 0.12 } $ & $3.84_{ \pm 0.20 }$ \\
 \multicolumn{1}{c}{}     &                    &                  &                   &                  \\
 \multicolumn{1}{c}{Ask4} &                    &                  &                   &                  \\ \midrule
Baseline   & $1.00_{ \pm 0.00 } $ & $1.00_{ \pm 0.00 }$   &    $3.03_{ \pm 0.06 } $ & $3.05_{ \pm 0.03 }$ \\
Ours(v)    & $2.13_{ \pm 0.05 } $ & $2.10_{ \pm 0.04 }$   &    $3.44_{ \pm 0.24 } $ & $3.47_{ \pm 0.22 }$ \\
Ours(num)  & $1.56_{ \pm 0.03 } $ & $1.60_{ \pm 0.08 }$   &    $3.12_{ \pm 0.09 } $ & $3.09_{ \pm 0.05 }$ \\
Ours(nu)   & $1.56_{ \pm 0.04 } $ & $1.59_{ \pm 0.05 }$   &    $3.19_{ \pm 0.08 } $ & $3.13_{ \pm 0.06 }$ \\
Ours(full) & $1.49_{ \pm 0.02 } $ & $1.54_{ \pm 0.05 }$   &    $3.06_{ \pm 0.08 } $ & $3.06_{ \pm 0.04 }$ \\
 \bottomrule
 \end{tabularx}
  \caption{Question vocabulary for comparative models presented in Tab.~\redr{2}.
    Here, $n_{\mathrm{vocab}}$ shows the average vocabulary size of the questions,
    and $\overline{n}_{\mathrm{vocab}}$, which shows the average vocabulary size of the dialogues.
  % \txtodo{Add definitions of question mean and diglogue mean.}
}\label{tab:results_vocab}
\end{centering}
% \vspace{-1em}
\end{table}
